Priced, not passed: what accounting agents actually lose in a SPED-native audit environment

Agent evaluations usually score tasks as passed or failed, while economic errors are priced asymmetrically in currency. malha generates a synthetic Brazilian company's complete fiscal year---NF-e XMLs, double-entry journal, trial balances, rendered scanned source documents, and statutory ECD and EFD-Contribui\c{c}\~oes filings---injects defects from a frozen taxonomy, re-derives downstream artifacts for consistency, and prices an agent's audit in expected statutory loss under Lei 8.218/1991. The oracle recomputes artifact evidence rather than trusting agent output. Three studies are reported. v1 rows are exploratory because the pre-correction filesystem exposed defect metadata in world.json. In corrected v2/v2.1, deterministic-first architecture, a read-only SQL index, a fail-closed ledger, and scan pixels improve hybrid agents over the original malha_rules floor, but a stronger deterministic floor, ocr_rules_book4, remains cheaper than every measured agent. v2.2 regenerates the pool with a defect-independent scan inventory, adds stateless transcription floors and a rules-plus-agent hybrid, and is explicitly exploratory because its oracle guard failed even though every registered cell completed. On that pool, earlier scan claims did not replicate, the hybrid's apparent mean advantage is fragile and driven by many false positives, and a VLM-transcriber-plus-rules pipeline is cheaper than the hybrid. On a subtle-wording slice, the registered H5 contrast favors the text agent, but the margin is dominated by one delivery-stamp date-format class rather than semantic wording; without that class the contrast is not resolved. Overall, malha does not show agents exceeding strong deterministic automation. Separate 8B SFT/GRPO results are diagnostic only.

==> tables/v22_api_costs.tex <==
% auto-generated by scripts/build_v22_paper.py from results/v22/analysis.json (api_costs), results/v22/vlm_ocr_shards/USAGE_REPORT.json, results/v22/episodes_frontier.jsonl — do not hand-edit (measured tokens x list price (glm-flash 0.15/0.5 USD per 1M in/out); subscription key, so this is not an invoice; quota-error rows carry no usage)
\begin{tabular}{lp{5.2cm}lrrrrr}
\toprule
pool & arm & noise & billed rows & in (M tok) & out (M tok) & USD & USD/world \\
\midrule
v22 & \texttt{agent\_v2\_fixed+glm-flash} & clean & 60 & 11.85 & 0.21 & 1.89 & 0.031 \\
v22 & \texttt{agent\_v2\_fixed+glm-flash} & noisy\_scan & 60 & 11.55 & 1.02 & 2.24 & 0.037 \\
v22 & \texttt{agent\_v2\_vlm+glm-flash} & noisy\_scan & 60 & 11.24 & 0.96 & 2.16 & 0.036 \\
v22 & \texttt{agent\_v2\_vlm\_book4+glm-flash} & noisy\_scan & 60 & 14.98 & 0.89 & 2.69 & 0.045 \\
v22\_subtle & \texttt{agent\_v2\_fixed+glm-flash} & clean & 30 & 5.13 & 0.35 & 0.95 & 0.032 \\
v22 & VLM transcription (\texttt{ocr\_rules*\_vlm}), cache incomplete, arm not scored & mild\_scan & 569 & 1.29 & 0.22 & 0.30 & -- \\
v22 & VLM transcription (\texttt{ocr\_rules*\_vlm}) & noisy\_scan & 1200 & 2.72 & 0.44 & 0.63 & 0.010 \\
legacy\_v2 & VLM transcription (\texttt{ocr\_rules*\_vlm}) & mild\_scan & 593 & 1.06 & 0.17 & 0.25 & 0.008 \\
legacy\_v2 & VLM transcription (\texttt{ocr\_rules*\_vlm}) & noisy\_scan & 593 & 1.06 & 0.20 & 0.26 & 0.009 \\
v22\_subtle & VLM transcription (\texttt{ocr\_rules*\_vlm}) & mild\_scan & 600 & 1.36 & 0.23 & 0.32 & 0.011 \\
v22\_subtle & VLM transcription (\texttt{ocr\_rules*\_vlm}), cache incomplete, arm not scored & noisy\_scan & 535 & 1.22 & 0.21 & 0.29 & -- \\
v22 & \texttt{agent\_v2\_ledger+deepseek} & noisy\_scan & 7 & 1.77 & 0.13 & no list price & -- \\
\midrule \multicolumn{6}{l}{total at list price, priced rows only} & 11.97 &  \\
\bottomrule
\end{tabular}


==> tables/v22_completeness.tex <==
% auto-generated by scripts/build_v22_paper.py from results/v22/analysis_posthoc.json (post hoc; not registered readings) — do not hand-edit (agent cells and every incomplete cell; complete floor cells omitted)
\begin{tabular}{lllrrlp{4.5cm}}
\toprule
pool & arm & noise & worlds done/planned & episodes & missing because & missing seeds \\
\midrule
legacy\_v2 & \texttt{agent\_v1+glm-flash} & clean & 30/30 & 90 & -- & -- \\
legacy\_v2 & \texttt{agent\_v2\_fixed+deepseek-flash} & clean & 30/30 & 90 & -- & -- \\
legacy\_v2 & \texttt{agent\_v2\_fixed+deepseek-flash} & mild\_scan & 30/30 & 90 & -- & -- \\
legacy\_v2 & \texttt{agent\_v2\_fixed+deepseek-flash} & noisy\_scan & 30/30 & 90 & -- & -- \\
legacy\_v2 & \texttt{agent\_v2\_fixed+glm-flash} & clean & 30/30 & 90 & -- & -- \\
legacy\_v2 & \texttt{agent\_v2\_fixed+glm-flash} & mild\_scan & 30/30 & 90 & -- & -- \\
legacy\_v2 & \texttt{agent\_v2\_fixed+glm-flash} & noisy\_scan & 30/30 & 90 & -- & -- \\
legacy\_v2 & \texttt{agent\_v2\_vlm+glm-flash} & clean & 30/30 & 90 & -- & -- \\
legacy\_v2 & \texttt{agent\_v2\_vlm+glm-flash} & mild\_scan & 30/30 & 90 & -- & -- \\
legacy\_v2 & \texttt{agent\_v2\_vlm+glm-flash} & noisy\_scan & 30/30 & 90 & -- & -- \\
v22\_subtle & \texttt{agent\_v2\_fixed+glm-flash} & clean & 30/30 & 30 & -- & -- \\
v22 & \texttt{agent\_v2\_fixed+glm-flash} & clean & 60/60 & 60 & -- & -- \\
v22 & \texttt{agent\_v2\_fixed+glm-flash} & noisy\_scan & 60/60 & 60 & -- & -- \\
v22 & \texttt{agent\_v2\_vlm+glm-flash} & noisy\_scan & 60/60 & 60 & -- & -- \\
v22 & \texttt{agent\_v2\_vlm\_book4+glm-flash} & noisy\_scan & 60/60 & 60 & -- & -- \\
v22\_subtle & VLM transcripts for \texttt{ocr\_rules*\_vlm} & noisy\_scan & 535/600 scans & 0 & cache incomplete, arm not scored & -- \\
v22 & VLM transcripts for \texttt{ocr\_rules*\_vlm} & mild\_scan & 569/1200 scans & 0 & cache incomplete, arm not scored & -- \\
\bottomrule
\end{tabular}


==> tables/v22_contrasts.tex <==
% auto-generated by scripts/build_v22_paper.py from results/v22/registered_analysis.json, results/v22/analysis.json — do not hand-edit
\begin{tabular}{lrrrrrrl}
\toprule
contrast $A-B$ (positive: $B$ cheaper) & $\Delta$EL [95\% CI], BRL & BCa 95\% & under \texttt{strict\_cap3} & Holm $p$ & worlds $B$ / $A$ cheaper / tied (sign $p$) & worlds & reading \\
\midrule
H1: \texttt{ocr\_rules\_book4} $-$ \texttt{agent\_v2\_vlm\_book4+glm-flash}, v22 noisy\_scan & $+679$ [$-95$, $+1{,}609$] & [$+8$, $+1{,}829$] & $+679$ [$-95$, $+1{,}609$] & primary & 9 / 45 / 6 ($7\times10^{-7}$) & 60/60 & not resolved; exploratory; fragile \\
H2: \texttt{agent\_v2\_vlm+glm-flash} $-$ \texttt{ocr\_rules\_book4\_vlm}, v22 noisy\_scan & $+6{,}777$ [$+4{,}155$, $+9{,}851$] & [$+4{,}472$, $+10{,}563$] & $+6{,}826$ [$+4{,}213$, $+9{,}917$] & 0.0004 & 53 / 0 / 7 ($2\times10^{-16}$) & 60/60 & supported; exploratory \\
H3: \texttt{agent\_v2\_fixed+glm-flash} $-$ \texttt{agent\_v2\_vlm+glm-flash}, v22 noisy\_scan, scan-class slice & $-3$ [$-1{,}904$, $+2{,}051$] & [$-1{,}880$, $+2{,}082$] & $-23$ [$-1{,}930$, $+2{,}009$] & 0.9984 & 20 / 21 / 19 (1.000) & 60/60 & not resolved; exploratory; fragile \\
H4: \texttt{ocr\_rules\_book4\_reocr} $-$ \texttt{ocr\_rules\_book4\_deskew}, v22 noisy\_scan & $+2{,}456$ [$+919$, $+4{,}370$] & [$+1{,}168$, $+4{,}979$] & $+2{,}456$ [$+919$, $+4{,}370$] & 0.0004 & 20 / 1 / 39 ($2\times10^{-5}$) & 60/60 & supported; exploratory \\
H5: \texttt{ocr\_rules\_book4} $-$ \texttt{agent\_v2\_fixed+glm-flash}, v22\_subtle clean & $+7{,}514$ [$+3{,}481$, $+11{,}841$] & [$+3{,}780$, $+12{,}222$] & $+7{,}143$ [$+3{,}076$, $+11{,}486$] & 0.0020 & 18 / 12 / 0 (0.362) & 30/30 & supported; exploratory \\
\midrule \multicolumn{7}{l}{\emph{Post hoc contrasts, confirmatory pool, \texttt{noisy\_scan} (not registered)}} \\
\texttt{agent\_v2\_fixed+glm-flash} $-$ \texttt{agent\_v2\_vlm+glm-flash} (H3 pair, outside its registered cell or slice) & $+40$ [$-2{,}070$, $+2{,}212$] & [$-2{,}130$, $+2{,}151$] & $+20$ [$-2{,}096$, $+2{,}190$] & -- & 23 / 26 / 11 (0.775) & 60/60 & post hoc \\
\texttt{agent\_v2\_vlm+glm-flash} $-$ \texttt{agent\_v2\_vlm\_book4+glm-flash} & $+3{,}623$ [$+800$, $+6{,}764$] & [$+1{,}145$, $+7{,}362$] & $+3{,}672$ [$+853$, $+6{,}807$] & -- & 27 / 21 / 12 (0.471) & 60/60 & post hoc \\
\texttt{malha\_rules\_book4} $-$ \texttt{ocr\_rules\_book4} & $+6{,}197$ [$+3{,}655$, $+9{,}206$] & [$+3{,}941$, $+9{,}800$] & $+6{,}197$ [$+3{,}655$, $+9{,}206$] & -- & 32 / 9 / 19 ($4\times10^{-4}$) & 60/60 & post hoc \\
\texttt{malha\_rules} $-$ \texttt{agent\_v2\_fixed+glm-flash} & $+5{,}270$ [$+3{,}034$, $+7{,}676$] & [$+3{,}279$, $+8{,}019$] & $+5{,}241$ [$+3{,}014$, $+7{,}640$] & -- & 32 / 25 / 3 (0.427) & 60/60 & post hoc \\
\texttt{malha\_rules} $-$ \texttt{agent\_v2\_vlm+glm-flash} & $+5{,}310$ [$+3{,}099$, $+7{,}766$] & [$+3{,}282$, $+7{,}996$] & $+5{,}260$ [$+3{,}054$, $+7{,}715$] & -- & 28 / 29 / 3 (1.000) & 60/60 & post hoc \\
\texttt{malha\_rules} $-$ \texttt{agent\_v2\_vlm\_book4+glm-flash} & $+8{,}933$ [$+6{,}007$, $+12{,}247$] & [$+6{,}334$, $+12{,}859$] & $+8{,}933$ [$+6{,}007$, $+12{,}247$] & -- & 40 / 18 / 2 (0.005) & 60/60 & post hoc \\
\texttt{malha\_rules} $-$ \texttt{ocr\_rules\_book4} & $+8{,}254$ [$+5{,}395$, $+11{,}543$] & [$+5{,}677$, $+12{,}080$] & $+8{,}254$ [$+5{,}395$, $+11{,}543$] & -- & 41 / 6 / 13 ($2\times10^{-7}$) & 60/60 & post hoc \\
\texttt{ocr\_rules\_book4\_deskew} $-$ \texttt{agent\_v2\_fixed+glm-flash} & $-5{,}439$ [$-8{,}458$, $-2{,}881$] & [$-9{,}111$, $-3{,}221$] & $-5{,}468$ [$-8{,}482$, $-2{,}910$] & -- & 2 / 49 / 9 ($1\times10^{-12}$) & 60/60 & post hoc \\
\texttt{ocr\_rules\_book4\_deskew} $-$ \texttt{agent\_v2\_vlm+glm-flash} & $-5{,}400$ [$-8{,}492$, $-2{,}674$] & [$-9{,}036$, $-2{,}962$] & $-5{,}449$ [$-8{,}539$, $-2{,}723$] & -- & 2 / 50 / 8 ($6\times10^{-13}$) & 60/60 & post hoc \\
\texttt{ocr\_rules\_book4\_deskew} $-$ \texttt{agent\_v2\_vlm\_book4+glm-flash} & $-1{,}776$ [$-3{,}728$, $-227$] & [$-4{,}333$, $-494$] & $-1{,}776$ [$-3{,}728$, $-227$] & -- & 3 / 51 / 6 ($3\times10^{-12}$) & 60/60 & post hoc \\
\texttt{ocr\_rules\_book4\_deskew} $-$ \texttt{ocr\_rules\_book4\_vlm} & $+1{,}377$ [$+414$, $+2{,}533$] & [$+573$, $+2{,}844$] & $+1{,}377$ [$+414$, $+2{,}533$] & -- & 8 / 0 / 52 (0.008) & 60/60 & post hoc \\
\texttt{ocr\_rules\_book4} $-$ \texttt{agent\_v2\_fixed+glm-flash} (H5 pair, outside its registered cell or slice) & $-2{,}983$ [$-5{,}589$, $-972$] & [$-6{,}588$, $-1{,}275$] & $-3{,}013$ [$-5{,}621$, $-998$] & -- & 7 / 41 / 12 ($6\times10^{-7}$) & 60/60 & post hoc \\
\texttt{ocr\_rules\_book4} $-$ \texttt{agent\_v2\_vlm+glm-flash} & $-2{,}944$ [$-5{,}981$, $-258$] & [$-6{,}522$, $-548$] & $-2{,}993$ [$-6{,}022$, $-303$] & -- & 9 / 43 / 8 ($2\times10^{-6}$) & 60/60 & post hoc \\
\texttt{ocr\_rules\_book4} $-$ \texttt{ocr\_rules\_book4\_vlm} & $+3{,}833$ [$+2{,}063$, $+5{,}931$] & [$+2{,}277$, $+6{,}400$] & $+3{,}833$ [$+2{,}063$, $+5{,}931$] & -- & 27 / 0 / 33 ($1\times10^{-8}$) & 60/60 & post hoc \\
\texttt{ocr\_rules\_book4\_reocr} $-$ \texttt{ocr\_rules\_book4} & $+0$ [$+0$, $+0$] & -- & $+0$ [$+0$, $+0$] & -- & 0 / 0 / 60 (--) & 60/60 & post hoc \\
\texttt{ocr\_rules\_book4\_vlm} $-$ \texttt{agent\_v2\_fixed+glm-flash} & $-6{,}816$ [$-9{,}989$, $-4{,}221$] & [$-10{,}586$, $-4{,}508$] & $-6{,}845$ [$-10{,}016$, $-4{,}245$] & -- & 0 / 51 / 9 ($9\times10^{-16}$) & 60/60 & post hoc \\
\texttt{ocr\_rules\_book4\_vlm} $-$ \texttt{agent\_v2\_vlm\_book4+glm-flash} & $-3{,}153$ [$-5{,}167$, $-1{,}513$] & [$-5{,}787$, $-1{,}750$] & $-3{,}153$ [$-5{,}167$, $-1{,}513$] & -- & 0 / 54 / 6 ($1\times10^{-16}$) & 60/60 & post hoc \\
\texttt{ocr\_rules} $-$ \texttt{agent\_v2\_fixed+glm-flash} & $-927$ [$-3{,}533$, $+1{,}145$] & [$-4{,}381$, $+792$] & $-957$ [$-3{,}558$, $+1{,}119$] & -- & 13 / 38 / 9 ($6\times10^{-4}$) & 60/60 & post hoc \\
\texttt{ocr\_rules} $-$ \texttt{agent\_v2\_vlm+glm-flash} & $-888$ [$-3{,}896$, $+1{,}824$] & [$-4{,}417$, $+1{,}501$] & $-937$ [$-3{,}948$, $+1{,}779$] & -- & 13 / 38 / 9 ($6\times10^{-4}$) & 60/60 & post hoc \\
\texttt{ocr\_rules} $-$ \texttt{agent\_v2\_vlm\_book4+glm-flash} & $+2{,}735$ [$+1{,}296$, $+4{,}428$] & [$+1{,}438$, $+4{,}707$] & $+2{,}735$ [$+1{,}296$, $+4{,}428$] & -- & 20 / 35 / 5 (0.058) & 60/60 & post hoc \\
\bottomrule
\end{tabular}


==> tables/v22_cost_detail.tex <==
% auto-generated by scripts/build_v22_paper.py from results/v22/analysis_posthoc.json (post hoc; not registered readings) — do not hand-edit (measured tokens x list price; subscription key, not an invoice)
\begin{tabular}{lllrrrrrlrr}
\toprule
pool & arm & noise & worlds & USD/world & tokens in / out per episode & requests / tool calls per episode & wall s/episode & against floor & extra TP / FP & $\Delta$EL BRL/world (positive: agent cheaper) \\
\midrule
v22\_subtle & \texttt{agent\_v2\_fixed+glm-flash} & clean & 30 & 0.032 & 171k / 12k & 12.3 / 25.0 & 141 & \texttt{ocr\_rules\_book4} & +31 / +45 & $+7{,}514$ \\
v22\_subtle & \texttt{agent\_v2\_fixed+glm-flash} & clean & 30 & 0.032 & 171k / 12k & 12.3 / 25.0 & 141 & \texttt{ocr\_rules\_book4\_deskew} & +32 / +45 & $+8{,}030$ \\
v22\_subtle & \texttt{agent\_v2\_fixed+glm-flash} & clean & 30 & 0.032 & 171k / 12k & 12.3 / 25.0 & 141 & \texttt{ocr\_rules\_book4\_vlm} & -- & -- \\
v22 & \texttt{agent\_v2\_fixed+glm-flash} & clean & 60 & 0.031 & 198k / 4k & 16.6 / 25.0 & 110 & \texttt{ocr\_rules\_book4} & -29 / +94 & $-6{,}452$ \\
v22 & \texttt{agent\_v2\_fixed+glm-flash} & clean & 60 & 0.031 & 198k / 4k & 16.6 / 25.0 & 110 & \texttt{ocr\_rules\_book4\_deskew} & -9 / +94 & $-1{,}851$ \\
v22 & \texttt{agent\_v2\_fixed+glm-flash} & clean & 60 & 0.031 & 198k / 4k & 16.6 / 25.0 & 110 & \texttt{ocr\_rules\_book4\_vlm} & -- & -- \\
v22 & \texttt{agent\_v2\_fixed+glm-flash} & noisy\_scan & 60 & 0.037 & 193k / 17k & 10.9 / 25.1 & 183 & \texttt{ocr\_rules\_book4} & -13 / +60 & $-2{,}983$ \\
v22 & \texttt{agent\_v2\_fixed+glm-flash} & noisy\_scan & 60 & 0.037 & 193k / 17k & 10.9 / 25.1 & 183 & \texttt{ocr\_rules\_book4\_deskew} & -25 / +75 & $-5{,}439$ \\
v22 & \texttt{agent\_v2\_fixed+glm-flash} & noisy\_scan & 60 & 0.037 & 193k / 17k & 10.9 / 25.1 & 183 & \texttt{ocr\_rules\_book4\_vlm} & -33 / +75 & $-6{,}816$ \\
v22 & \texttt{agent\_v2\_vlm+glm-flash} & noisy\_scan & 60 & 0.036 & 187k / 16k & 10.7 / 25.0 & 186 & \texttt{ocr\_rules\_book4} & -16 / +79 & $-2{,}944$ \\
v22 & \texttt{agent\_v2\_vlm+glm-flash} & noisy\_scan & 60 & 0.036 & 187k / 16k & 10.7 / 25.0 & 186 & \texttt{ocr\_rules\_book4\_deskew} & -28 / +94 & $-5{,}400$ \\
v22 & \texttt{agent\_v2\_vlm+glm-flash} & noisy\_scan & 60 & 0.036 & 187k / 16k & 10.7 / 25.0 & 186 & \texttt{ocr\_rules\_book4\_vlm} & -36 / +94 & $-6{,}777$ \\
v22 & \texttt{agent\_v2\_vlm\_book4+glm-flash} & noisy\_scan & 60 & 0.045 & 250k / 15k & 12.6 / 24.8 & 188 & \texttt{ocr\_rules\_book4} & +9 / +123 & $+679$ \\
v22 & \texttt{agent\_v2\_vlm\_book4+glm-flash} & noisy\_scan & 60 & 0.045 & 250k / 15k & 12.6 / 24.8 & 188 & \texttt{ocr\_rules\_book4\_deskew} & -3 / +138 & $-1{,}776$ \\
v22 & \texttt{agent\_v2\_vlm\_book4+glm-flash} & noisy\_scan & 60 & 0.045 & 250k / 15k & 12.6 / 24.8 & 188 & \texttt{ocr\_rules\_book4\_vlm} & -11 / +138 & $-3{,}153$ \\
legacy\_v2 & VLM transcription & mild\_scan & -- & 0.008 & 1.06M / 0.17M total & 593 requests total & -- & -- & -- & -- \\
legacy\_v2 & VLM transcription & noisy\_scan & -- & 0.009 & 1.06M / 0.20M total & 593 requests total & -- & -- & -- & -- \\
v22\_subtle & VLM transcription & mild\_scan & -- & 0.011 & 1.36M / 0.23M total & 600 requests total & -- & -- & -- & -- \\
v22\_subtle & VLM transcription (incomplete) & noisy\_scan & -- & -- & 1.22M / 0.21M total & 535 requests total & -- & -- & -- & -- \\
v22 & VLM transcription (incomplete) & mild\_scan & -- & -- & 1.29M / 0.22M total & 569 requests total & -- & -- & -- & -- \\
v22 & VLM transcription & noisy\_scan & -- & 0.011 & 2.72M / 0.44M total & 1200 requests total & -- & -- & -- & -- \\
\bottomrule
\end{tabular}


==> tables/v22_design.tex <==
% auto-generated by scripts/build_v22_paper.py from results/v22/prereg_v3_provenance.json, results/v22/pool/*/POOL_MANIFEST.json, results/v22/registered_analysis.json, results/v22/analysis.json — do not hand-edit (tag prereg-v3 -> commit 23e95a464fa9, tagged 2026-11-30T06:19:23Z; registration sha256 c64e08742ec148a1)
\begin{tabular}{lllllllp{4.6cm}p{3.2cm}}
\toprule
regime & seeds & worlds & \texttt{gen\_version} & Tesseract & oracle gate & inventory gate & agent cells with rows (worlds done/planned, $k{=}1$) & status \\
\midrule
confirmatory pool & 601--660 & 60 & 2.2 & 5.5.5 & 121/123 \textbf{fail} & pass & \texttt{fixed} clean 60/60; \texttt{fixed} noisy\_scan 60/60; \texttt{vlm} noisy\_scan 60/60; \texttt{vlm\_book4} noisy\_scan 60/60 & registered; guard 6.1 failed, so exploratory \\
subtle slice & 701--730 & 30 & 2.2 & 5.5.5 & 75/75 pass & pass & \texttt{fixed} clean 30/30 & registered \\
legacy locked pool & 501--530 & 30 & 2.0 & -- & -- & -- & none new & exploratory (D049, D051) \\
\midrule \multicolumn{9}{l}{Registration: tag \texttt{prereg-v3} at commit \texttt{23e95a464fa9}, tagged 2026-11-30 06:19:23 UTC; local tag, not pushed at tagging.} \\
\bottomrule
\end{tabular}


==> tables/v22_floor_matrix.tex <==
% auto-generated by scripts/build_v22_paper.py from results/v22/analysis_posthoc.json (post hoc; not registered readings) — do not hand-edit (pool v22, noisy_scan; cell: Delta EL [95% CI]; worlds agent cheaper / floor cheaper / tied; bold: interval excludes 0; positive: agent cheaper)
\begin{tabular}{lrrrr}
\toprule
floor (most expensive first) & floor mean EL, all worlds & floor $-$ \texttt{agent\_v2\_fixed+glm-flash} & floor $-$ \texttt{agent\_v2\_vlm+glm-flash} & floor $-$ \texttt{agent\_v2\_vlm\_book4+glm-flash} \\
\midrule
\texttt{flag\_everything} & 31,180 & \textbf{$+23{,}682$ [$+19{,}225$, $+28{,}334$]; 60 / 0 / 0} & \textbf{$+23{,}722$ [$+19{,}089$, $+28{,}502$]; 60 / 0 / 0} & \textbf{$+27{,}345$ [$+22{,}208$, $+32{,}945$]; 60 / 0 / 0} \\
\texttt{file\_as\_is} & 26,430 & \textbf{$+18{,}932$ [$+14{,}475$, $+23{,}584$]; 48 / 11 / 1} & \textbf{$+18{,}972$ [$+14{,}339$, $+23{,}752$]; 46 / 13 / 1} & \textbf{$+22{,}595$ [$+17{,}458$, $+28{,}195$]; 53 / 7 / 0} \\
\texttt{malha\_rules} & 12,768 & \textbf{$+5{,}270$ [$+3{,}034$, $+7{,}676$]; 32 / 25 / 3} & \textbf{$+5{,}310$ [$+3{,}099$, $+7{,}766$]; 28 / 29 / 3} & \textbf{$+8{,}933$ [$+6{,}007$, $+12{,}247$]; 40 / 18 / 2} \\
\texttt{malha\_rules\_book4} & 10,712 & \textbf{$+3{,}214$ [$+908$, $+5{,}690$]; 25 / 30 / 5} & \textbf{$+3{,}254$ [$+946$, $+5{,}781$]; 24 / 33 / 3} & \textbf{$+6{,}877$ [$+4{,}233$, $+9{,}957$]; 34 / 23 / 3} \\
\texttt{ocr\_rules} & 6,571 & $-927$ [$-3{,}533$, $+1{,}145$]; 13 / 38 / 9 & $-888$ [$-3{,}896$, $+1{,}824$]; 13 / 38 / 9 & \textbf{$+2{,}735$ [$+1{,}296$, $+4{,}428$]; 20 / 35 / 5} \\
\texttt{ocr\_rules\_reocr} & 6,571 & $-927$ [$-3{,}533$, $+1{,}145$]; 13 / 38 / 9 & $-888$ [$-3{,}896$, $+1{,}824$]; 13 / 38 / 9 & \textbf{$+2{,}735$ [$+1{,}296$, $+4{,}428$]; 20 / 35 / 5} \\
\texttt{ocr\_rules\_book4} & 4,514 & \textbf{$-2{,}983$ [$-5{,}589$, $-972$]; 7 / 41 / 12} & \textbf{$-2{,}944$ [$-5{,}981$, $-258$]; 9 / 43 / 8} & $+679$ [$-95$, $+1{,}609$]; 9 / 45 / 6 \\
\texttt{ocr\_rules\_book4\_reocr} & 4,514 & \textbf{$-2{,}983$ [$-5{,}589$, $-972$]; 7 / 41 / 12} & \textbf{$-2{,}944$ [$-5{,}981$, $-258$]; 9 / 43 / 8} & $+679$ [$-95$, $+1{,}609$]; 9 / 45 / 6 \\
\texttt{ocr\_rules\_deskew} & 4,115 & \textbf{$-3{,}383$ [$-6{,}426$, $-769$]; 7 / 45 / 8} & \textbf{$-3{,}343$ [$-6{,}462$, $-580$]; 7 / 47 / 6} & $+280$ [$-2{,}107$, $+2{,}477$]; 17 / 40 / 3 \\
\texttt{ocr\_rules\_vlm} & 2,738 & \textbf{$-4{,}760$ [$-8{,}030$, $-2{,}005$]; 5 / 47 / 8} & \textbf{$-4{,}721$ [$-7{,}896$, $-2{,}001$]; 5 / 49 / 6} & $-1{,}097$ [$-3{,}578$, $+1{,}226$]; 13 / 43 / 4 \\
\texttt{ocr\_rules\_book4\_deskew} & 2,059 & \textbf{$-5{,}439$ [$-8{,}458$, $-2{,}881$]; 2 / 49 / 9} & \textbf{$-5{,}400$ [$-8{,}492$, $-2{,}674$]; 2 / 50 / 8} & \textbf{$-1{,}776$ [$-3{,}728$, $-227$]; 3 / 51 / 6} \\
\texttt{ocr\_rules\_book4\_vlm} & 682 & \textbf{$-6{,}816$ [$-9{,}989$, $-4{,}221$]; 0 / 51 / 9} & \textbf{$-6{,}777$ [$-9{,}849$, $-4{,}153$]; 0 / 53 / 7} & \textbf{$-3{,}153$ [$-5{,}167$, $-1{,}513$]; 0 / 54 / 6} \\
\bottomrule
\end{tabular}


==> tables/v22_floor_matrix_subtle.tex <==
% auto-generated by scripts/build_v22_paper.py from results/v22/analysis_posthoc.json (post hoc; not registered readings) — do not hand-edit (pool v22_subtle, clean; cell: Delta EL [95% CI]; worlds agent cheaper / floor cheaper / tied; bold: interval excludes 0; positive: agent cheaper)
\begin{tabular}{lrr}
\toprule
floor (most expensive first) & floor mean EL, all worlds & floor $-$ \texttt{agent\_v2\_fixed+glm-flash} \\
\midrule
\texttt{flag\_everything} & 28,367 & \textbf{$+20{,}455$ [$+15{,}270$, $+26{,}208$]; 30 / 0 / 0} \\
\texttt{file\_as\_is} & 23,617 & \textbf{$+15{,}705$ [$+10{,}520$, $+21{,}458$]; 25 / 5 / 0} \\
\texttt{malha\_rules} & 17,230 & \textbf{$+9{,}318$ [$+5{,}558$, $+13{,}292$]; 21 / 9 / 0} \\
\texttt{ocr\_rules\_deskew} & 17,230 & \textbf{$+9{,}318$ [$+5{,}558$, $+13{,}292$]; 21 / 9 / 0} \\
\texttt{ocr\_rules} & 16,713 & \textbf{$+8{,}801$ [$+5{,}043$, $+12{,}868$]; 20 / 10 / 0} \\
\texttt{ocr\_rules\_reocr} & 16,713 & \textbf{$+8{,}801$ [$+5{,}043$, $+12{,}868$]; 20 / 10 / 0} \\
\texttt{malha\_rules\_book4} & 15,942 & \textbf{$+8{,}030$ [$+4{,}055$, $+12{,}344$]; 19 / 11 / 0} \\
\texttt{ocr\_rules\_book4\_deskew} & 15,942 & \textbf{$+8{,}030$ [$+4{,}055$, $+12{,}344$]; 19 / 11 / 0} \\
\texttt{ocr\_rules\_book4} & 15,426 & \textbf{$+7{,}514$ [$+3{,}481$, $+11{,}841$]; 18 / 12 / 0} \\
\texttt{ocr\_rules\_book4\_reocr} & 15,426 & \textbf{$+7{,}514$ [$+3{,}481$, $+11{,}841$]; 18 / 12 / 0} \\
\bottomrule
\end{tabular}


==> tables/v22_frontier.tex <==
% auto-generated by scripts/build_v22_paper.py from results/v22/episodes_frontier.jsonl (exploratory lane, not registered) — do not hand-edit
\begin{tabular}{lllrrp{6cm}}
\toprule
arm & noise & worlds & mean EL (BRL) & FP/episode & status \\
\midrule
\texttt{agent\_v2\_ledger+deepseek} & noisy\_scan & 7/30 & 1,031 & 1.00 & incomplete: below the lane's own 27-world rule, no reading drawn \\
\texttt{agent\_v2\_sql+deepseek} & noisy\_scan & 0/30 & not run & -- & not run: no SQL-minus-ledger contrast, H2 of prereg-v2 untested \\
closed-lab frontier models & -- & 0 & not run & -- & not run: no credential (results/v22/frontier\_shards/STATUS.md) \\
\bottomrule
\end{tabular}


==> tables/v22_h5_classes.tex <==
% auto-generated by scripts/build_v22_h5.py from results/v22/h5_decomposition.json — do not hand-edit (per-class rows: PRE-REGISTRATION-V3 s.8, s.9.1; BRL per world over all worlds of the slice; descriptive, s.9.4)
\begin{tabular}{llrrrrrrrrr}
\toprule
class & kind & defects & exposure & floor TP & floor FP & agent TP & agent FP & recovered by agent & FP cost & $\Delta$ share \\
\midrule
\texttt{scan\_cutoff\_delivery} & date format (surface form) & 15 & $8{,}441$ & 0/15 & 0 & 15/15 & 0 & $+8{,}441$ & $+0$ & $+8{,}441$ \\
\texttt{scan\_personal\_expense} & semantic & 15 & $162$ & 0/15 & 0 & 14/15 & 1 & $+154$ & $-8$ & $+146$ \\
\texttt{scan\_ineligible\_credit\_desc} & semantic & 15 & $3{,}484$ & 0/15 & 0 & 4/15 & 5 & $+1{,}075$ & $-42$ & $+1{,}033$ \\
\texttt{expense\_personal\_mixed} & semantic & 15 & $3{,}323$ & 0/15 & 0 & 2/15 & 1 & $+24$ & $-8$ & $+15$ \\
\emph{semantic classes, total} & s.9.1 aggregate & 45 & $6{,}968$ & 0/45 & 0 & 20/45 & 7 & $+1{,}253$ & $-58$ & $+1{,}194$ \\
\texttt{cutoff\_violation} & not reworded & 1 & $849$ & 1/1 & 0 & 0/1 & 5 & $-849$ & $-42$ & $-890$ \\
\texttt{nfe\_value\_mismatch} & not reworded & 1 & $78$ & 1/1 & 0 & 1/1 & 11 & $+0$ & $-92$ & $-92$ \\
\texttt{pis\_cofins\_ineligible\_credit} & not reworded & 1 & $73$ & 1/1 & 0 & 0/1 & 16 & $-73$ & $-133$ & $-206$ \\
\texttt{scan\_value\_alteration} & not reworded & 1 & $517$ & 1/1 & 0 & 0/1 & 5 & $-517$ & $-42$ & $-558$ \\
\texttt{transitoria\_parking} & not reworded & 1 & $366$ & 1/1 & 0 & 0/1 & 1 & $-366$ & $-8$ & $-374$ \\
\emph{10 other classes, same counts in both arms} & not reworded & 10 & $6{,}325$ & 10/10 & 2 & 10/10 & 2 & $+0$ & $+0$ & $+0$ \\
\textbf{all classes (registered H5)} &  & 75 & $23{,}617$ & 15/75 & 2 & 46/75 & 47 & $+7{,}889$ & $-375$ & $+7{,}514$ \\
\bottomrule
\end{tabular}


==> tables/v22_h5_contrasts.tex <==
% auto-generated by scripts/build_v22_h5.py from results/v22/h5_decomposition.json — do not hand-edit (Delta = EL(floor) - EL(agent); every row but the first is post hoc)
\begin{tabular}{lrrrl}
\toprule
slice of the H5 contrast & $\Delta$EL [95\% CI], BRL & worlds & agent / floor cheaper / tied & status \\
\midrule
all classes (registered H5) & $+7{,}514$ [$+3{,}481$, $+11{,}841$] & 30 & 18 / 12 / 0 & registered \\
\texttt{scan\_cutoff\_delivery} only & $+8{,}441$ [$+4{,}940$, $+12{,}139$] & 30 & 15 / 0 / 15 & post hoc \\
all classes but \texttt{scan\_cutoff\_delivery} & $-927$ [$-3{,}455$, $+1{,}190$] & 30 & 11 / 18 / 1 & post hoc \\
the three semantic classes only & $+1{,}194$ [$+298$, $+2{,}326$] & 30 & 16 / 5 / 9 & post hoc \\
classes that were not reworded & $-2{,}121$ [$-4{,}366$, $-423$] & 30 & 0 / 23 / 7 & post hoc \\
worlds with a \texttt{scan\_cutoff\_delivery} defect, all classes & $+14{,}985$ [$+8{,}999$, $+20{,}831$] & 15 & 13 / 2 / 0 & post hoc \\
worlds without one, all classes & $+43$ [$-2{,}005$, $+2{,}180$] & 15 & 5 / 10 / 0 & post hoc \\
all but \texttt{scan\_cutoff\_delivery}; \texttt{aggressive}, FP R\$1{,}500 & $-3{,}584$ [$-10{,}239$, $+2{,}060$] & 30 & 7 / 22 / 1 & post hoc \\
all but \texttt{scan\_cutoff\_delivery}; \texttt{aggressive}, FP R\$250 & $-1{,}709$ [$-8{,}303$, $+3{,}804$] & 30 & 13 / 16 / 1 & post hoc \\
all but \texttt{scan\_cutoff\_delivery}; \texttt{conservative}, FP R\$1{,}500 & $-2{,}489$ [$-3{,}611$, $-1{,}438$] & 30 & 7 / 22 / 1 & post hoc \\
all but \texttt{scan\_cutoff\_delivery}; \texttt{conservative}, FP R\$250 & $-614$ [$-1{,}513$, $+147$] & 30 & 7 / 22 / 1 & post hoc \\
all but \texttt{scan\_cutoff\_delivery}; \texttt{neutral}, FP R\$1{,}500 & $-2{,}802$ [$-5{,}403$, $-489$] & 30 & 7 / 22 / 1 & post hoc \\
\bottomrule
\end{tabular}


==> tables/v22_h5_texture_fp.tex <==
% auto-generated by scripts/build_v22_h5.py from results/v22/h5_decomposition.json — do not hand-edit (false positives on benign texture, PRE-REGISTRATION-V3 s.9.3; counts over the cell)
\begin{tabular}{llrrrrrrrr}
\toprule
arm & noise & worlds & FP, all & decoy receipt & paraphrased DANFE & benign narration & benign stamp & on texture, same class & citing texture, any class \\
\midrule
\texttt{agent\_v2\_fixed+glm-flash} & clean & 30 & 47 & 0 & 3 & 1 & 0 & 4 & 13 \\
\texttt{file\_as\_is} & clean & 30 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{file\_as\_is} & mild\_scan & 30 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{file\_as\_is} & noisy\_scan & 30 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{flag\_everything} & clean & 30 & 570 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{flag\_everything} & mild\_scan & 30 & 570 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{flag\_everything} & noisy\_scan & 30 & 570 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{malha\_rules\_book4} & clean & 30 & 2 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{malha\_rules\_book4} & mild\_scan & 30 & 2 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{malha\_rules\_book4} & noisy\_scan & 30 & 2 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{malha\_rules} & clean & 30 & 2 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{malha\_rules} & mild\_scan & 30 & 2 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{malha\_rules} & noisy\_scan & 30 & 2 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{ocr\_rules\_book4\_deskew} & clean & 30 & 2 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{ocr\_rules\_book4\_deskew} & mild\_scan & 30 & 2 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{ocr\_rules\_book4\_deskew} & noisy\_scan & 30 & 2 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{ocr\_rules\_book4\_reocr} & clean & 30 & 2 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{ocr\_rules\_book4\_reocr} & mild\_scan & 30 & 2 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{ocr\_rules\_book4\_reocr} & noisy\_scan & 30 & 10 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{ocr\_rules\_book4\_vlm} & mild\_scan & 30 & 2 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{ocr\_rules\_book4} & clean & 30 & 2 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{ocr\_rules\_book4} & mild\_scan & 30 & 2 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{ocr\_rules\_book4} & noisy\_scan & 30 & 10 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{ocr\_rules\_deskew} & clean & 30 & 2 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{ocr\_rules\_deskew} & mild\_scan & 30 & 2 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{ocr\_rules\_deskew} & noisy\_scan & 30 & 2 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{ocr\_rules\_reocr} & clean & 30 & 2 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{ocr\_rules\_reocr} & mild\_scan & 30 & 2 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{ocr\_rules\_reocr} & noisy\_scan & 30 & 10 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{ocr\_rules\_vlm} & mild\_scan & 30 & 2 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{ocr\_rules} & clean & 30 & 2 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{ocr\_rules} & mild\_scan & 30 & 2 & 0 & 0 & 0 & 0 & 0 & 0 \\
\texttt{ocr\_rules} & noisy\_scan & 30 & 10 & 0 & 0 & 0 & 0 & 0 & 0 \\
\bottomrule
\end{tabular}


==> tables/v22_legacy_new_arms.tex <==
% auto-generated by scripts/build_v22_tables.py from results/v22/analysis.json — do not hand-edit (pool legacy_v2, gen_version 2.0,None)
\begin{tabular}{lllrrrr}
\toprule
arm & noise & status & mean EL (BRL) & worlds & \texttt{ocr\_rules\_book4} $-$ arm & \texttt{agent\_v2\_vlm+glm-flash} $-$ arm \\
\midrule
\texttt{ocr\_rules\_book4\_deskew} & clean & exploratory & 5,862 & 30 & -- & -- \\
\texttt{ocr\_rules\_book4\_deskew} & mild\_scan & exploratory & 3,705 & 30 & -- & -- \\
\texttt{ocr\_rules\_book4\_deskew} & noisy\_scan & exploratory & 3,705 & 30 & -- & -- \\
\texttt{ocr\_rules\_book4\_vlm} & clean & exploratory & not run & -- & -- & -- \\
\texttt{ocr\_rules\_book4\_vlm} & mild\_scan & exploratory & 108 & 30 & \textbf{+1,750 [+361, +3,500]} & \textbf{+6,339 [+3,748, +9,472]} \\
\texttt{ocr\_rules\_book4\_vlm} & noisy\_scan & exploratory & 474 & 30 & \textbf{+4,463 [+947, +9,601]} & \textbf{+5,511 [+2,765, +8,917]} \\
\texttt{agent\_v2\_vlm\_book4+glm-flash} & clean & exploratory & not run & -- & -- & -- \\
\texttt{agent\_v2\_vlm\_book4+glm-flash} & mild\_scan & exploratory & not run & -- & -- & -- \\
\texttt{agent\_v2\_vlm\_book4+glm-flash} & noisy\_scan & exploratory & not run & -- & -- & -- \\
\bottomrule
\end{tabular}


==> tables/v22_perworld.tex <==
% auto-generated by paper/build_v22_prose.py from results/v22/episodes_v22.jsonl, results/v22/registered_analysis.json, results/v2/analysis.json — do not hand-edit
\begin{tabular}{lrrrrrl}
\toprule
contrast $A-B$ & $\Delta$EL [95\% CI], BRL & worlds & $B$ cheaper & $A$ cheaper & tied & status \\
\midrule
H1: \texttt{ocr\_rules\_book4} $-$ \texttt{agent\_v2\_vlm\_book4+glm-flash} & +679 [$-$95, +1{,}609] & 60 & 9 & 45 & 6 & registered; exploratory \\
H2: \texttt{agent\_v2\_vlm+glm-flash} $-$ \texttt{ocr\_rules\_book4\_vlm} & +6{,}777 [+4{,}155, +9{,}851] & 60 & 53 & 0 & 7 & registered; exploratory \\
H3: \texttt{agent\_v2\_fixed+glm-flash} $-$ \texttt{agent\_v2\_vlm+glm-flash}, scan-class slice & $-$3 [$-$1{,}904, +2{,}051] & 60 & 20 & 21 & 19 & registered; exploratory \\
H4: \texttt{ocr\_rules\_book4\_reocr} $-$ \texttt{ocr\_rules\_book4\_deskew} & +2{,}456 [+919, +4{,}370] & 60 & 20 & 1 & 39 & registered; exploratory \\
\midrule
\texttt{ocr\_rules\_book4\_deskew} $-$ \texttt{agent\_v2\_vlm\_book4+glm-flash} & $-$1{,}776 [$-$3{,}728, $-$227] & 60 & 3 & 51 & 6 & post hoc \\
\texttt{ocr\_rules\_book4\_vlm} $-$ \texttt{agent\_v2\_vlm\_book4+glm-flash} & $-$3{,}153 [$-$5{,}167, $-$1{,}513] & 60 & 0 & 54 & 6 & post hoc \\
\texttt{ocr\_rules} $-$ \texttt{agent\_v2\_vlm+glm-flash} & $-$888 [$-$3{,}896, +1{,}824] & 60 & 13 & 38 & 9 & post hoc \\
\texttt{ocr\_rules} $-$ \texttt{agent\_v2\_fixed+glm-flash} & $-$927 [$-$3{,}533, +1{,}145] & 60 & 13 & 38 & 9 & post hoc \\
\texttt{agent\_v2\_fixed+glm-flash} $-$ \texttt{agent\_v2\_vlm+glm-flash} & +40 [$-$2{,}070, +2{,}212] & 60 & 23 & 26 & 11 & post hoc \\
\texttt{malha\_rules} $-$ \texttt{agent\_v2\_vlm+glm-flash} & +5{,}310 [+3{,}099, +7{,}766] & 60 & 28 & 29 & 3 & post hoc \\
\texttt{malha\_rules} $-$ \texttt{agent\_v2\_fixed+glm-flash} & +5{,}270 [+3{,}034, +7{,}676] & 60 & 32 & 25 & 3 & post hoc \\
\texttt{ocr\_rules\_book4} $-$ \texttt{agent\_v2\_vlm+glm-flash} & $-$2{,}944 [$-$5{,}981, $-$258] & 60 & 9 & 43 & 8 & post hoc \\
\texttt{ocr\_rules\_book4} $-$ \texttt{agent\_v2\_fixed+glm-flash} & $-$2{,}983 [$-$5{,}589, $-$972] & 60 & 7 & 41 & 12 & post hoc \\
\midrule
\multicolumn{7}{p{15.5cm}}{H1 in counts, over the 60 shared worlds: the hybrid adds 9 true positives and 123 false positives to the floor's findings; it never has fewer of either. Median per-world $\Delta$ $-$375; mean without the three largest differences +52; false-positive price at which the mean is zero: R\$581 (registered prices: R\$250 and R\$1{,}500).} \\
\bottomrule
\end{tabular}


==> tables/v22_primary_grid.tex <==
% auto-generated by scripts/build_v22_tables.py from results/v22/analysis.json — do not hand-edit (pool v22, gen_version 2.2, neutral_r250)
\begin{tabular}{lrrrrrr}
\toprule
arm & clean: mean EL [95\% CI] (BRL) & worlds$\times k$ & mild\_scan: mean EL [95\% CI] (BRL) & worlds$\times k$ & noisy\_scan: mean EL [95\% CI] (BRL) & worlds$\times k$ \\
\midrule
\texttt{file\_as\_is} & 26,430 [21,359, 32,011] & 60/60$\times$1 & 26,430 [21,359, 32,011] & 60/60$\times$1 & 26,430 [21,359, 32,011] & 60/60$\times$1 \\
\texttt{flag\_everything} & 31,180 [26,109, 36,761] & 60/60$\times$1 & 31,180 [26,109, 36,761] & 60/60$\times$1 & 31,180 [26,109, 36,761] & 60/60$\times$1 \\
\texttt{malha\_rules} & 12,768 [9,283, 16,519] & 60/60$\times$1 & 12,768 [9,283, 16,519] & 60/60$\times$1 & 12,768 [9,283, 16,519] & 60/60$\times$1 \\
\texttt{ocr\_rules} & 2,738 [1,208, 4,583] & 60/60$\times$1 & 6,202 [3,796, 8,946] & 60/60$\times$1 & 6,571 [4,217, 9,237] & 60/60$\times$1 \\
\texttt{malha\_rules\_book4} & 10,712 [7,432, 14,290] & 60/60$\times$1 & 10,712 [7,432, 14,290] & 60/60$\times$1 & 10,712 [7,432, 14,290] & 60/60$\times$1 \\
\texttt{ocr\_rules\_book4} & 682 [17, 1,691] & 60/60$\times$1 & 4,146 [2,064, 6,583] & 60/60$\times$1 & 4,514 [2,491, 6,866] & 60/60$\times$1 \\
\texttt{ocr\_rules\_book4\_deskew} & 5,283 [2,670, 8,464] & 60/60$\times$1 & 1,751 [555, 3,364] & 60/60$\times$1 & 2,059 [687, 3,788] & 60/60$\times$1 \\
\texttt{ocr\_rules\_book4\_vlm} & not run & -- & not run & -- & 682 [17, 1,691] & 60/60$\times$1 \\
\texttt{agent\_v2\_fixed+glm-flash} & 7,134 [4,450, 10,269] & 60/60$\times$1 & not run & -- & 7,498 [4,756, 10,746] & 60/60$\times$1 \\
\texttt{agent\_v2\_vlm+glm-flash} & not run & -- & not run & -- & 7,458 [4,648, 10,700] & 60/60$\times$1 \\
\texttt{agent\_v2\_vlm\_book4+glm-flash} & not run & -- & not run & -- & 3,835 [2,033, 6,014] & 60/60$\times$1 \\
\texttt{ocr\_rules\_book4\_reocr} & 1,756 [614, 3,280] & 60/60$\times$1 & 4,146 [2,064, 6,583] & 60/60$\times$1 & 4,514 [2,491, 6,866] & 60/60$\times$1 \\
\texttt{ocr\_rules\_deskew} & 7,339 [4,494, 10,634] & 60/60$\times$1 & 3,807 [1,992, 5,944] & 60/60$\times$1 & 4,115 [2,221, 6,317] & 60/60$\times$1 \\
\texttt{ocr\_rules\_reocr} & 3,812 [2,027, 5,939] & 60/60$\times$1 & 6,202 [3,796, 8,946] & 60/60$\times$1 & 6,571 [4,217, 9,237] & 60/60$\times$1 \\
\texttt{ocr\_rules\_vlm} & not run & -- & not run & -- & 2,738 [1,208, 4,583] & 60/60$\times$1 \\
\bottomrule
\end{tabular}


==> tables/v22_replication.tex <==
% auto-generated by paper/build_v22_prose.py from results/v22/episodes_v22.jsonl, results/v22/registered_analysis.json, results/v2/analysis.json — do not hand-edit
\begin{tabular}{p{5.2cm}rrrl}
\toprule
contrast $A-B$, \texttt{noisy\_scan} & legacy pool (v2.1), $k{=}3$ & regenerated pool (v2.2), $k{=}1$ & worlds & $A$ / $B$ cheaper \\
\midrule
\texttt{ocr\_rules} $-$ \texttt{agent\_v2\_vlm+glm-flash}, all classes & +5{,}084 [+1{,}476, +9{,}531] & $-$888 [$-$3{,}896, +1{,}824] & 60/60 & 38 / 13 \\
\texttt{agent\_v2\_fixed+glm-flash} $-$ \texttt{agent\_v2\_vlm+glm-flash}, scan-class slice (registered H3) & +2{,}163 [+157, +5{,}465] & $-$3 [$-$1{,}904, +2{,}051] & 60/60 & 21 / 20 \\
\texttt{agent\_v2\_fixed+glm-flash} $-$ \texttt{agent\_v2\_vlm+glm-flash}, all classes & +1{,}748 [$-$783, +5{,}294] & +40 [$-$2{,}070, +2{,}212] & 60/60 & 26 / 23 \\
\texttt{malha\_rules} $-$ \texttt{agent\_v2\_vlm+glm-flash}, all classes & +9{,}733 [+5{,}020, +15{,}080] & +5{,}310 [+3{,}099, +7{,}766] & 60/60 & 29 / 28 \\
\texttt{ocr\_rules\_book4} $-$ \texttt{agent\_v2\_vlm+glm-flash}, all classes & $-$1{,}048 [$-$5{,}437, +3{,}582] & $-$2{,}944 [$-$5{,}981, $-$258] & 60/60 & 43 / 9 \\
\bottomrule
\end{tabular}


==> tables/v22_scan_inventory.tex <==
% auto-generated by scripts/build_v22_paper.py from results/v22/design/scan_inventory_shape_*.json, oracle_gate_*.json, design files — do not hand-edit
\begin{tabular}{llp{7.2cm}ll}
\toprule
slice & noise & mean scan PNGs by number of scan-class defects (worlds) & receipt/DANFE/NFS-e/canhoto & oracle found/injected \\
\midrule
confirmatory & clean & 0: 20.0 ($n{=}10$); 1: 20.0 ($n{=}40$); 2: 20.0 ($n{=}10$) & 4/8/4/4 & 121/123 \\
confirmatory & mild\_scan & 0: 20.0 ($n{=}10$); 1: 20.0 ($n{=}40$); 2: 20.0 ($n{=}10$) & 4/8/4/4 & 121/123 \\
confirmatory & noisy\_scan & 0: 20.0 ($n{=}10$); 1: 20.0 ($n{=}40$); 2: 20.0 ($n{=}10$) & 4/8/4/4 & 121/123 \\
confirmatory & design & worlds per scan class: \texttt{cutoff\_delivery} 15, \texttt{ineligible\_credit\_desc} 15, \texttt{personal\_expense} 15, \texttt{value\_alteration} 15 &  & \textbf{fail}: seeds 635, 647 \\
subtle & clean & 1: 20.0 ($n{=}15$); 2: 20.0 ($n{=}14$); 3: 20.0 ($n{=}1$) & 4/8/4/4 & 75/75 \\
subtle & mild\_scan & 1: 20.0 ($n{=}15$); 2: 20.0 ($n{=}14$); 3: 20.0 ($n{=}1$) & 4/8/4/4 & 75/75 \\
subtle & noisy\_scan & 1: 20.0 ($n{=}15$); 2: 20.0 ($n{=}14$); 3: 20.0 ($n{=}1$) & 4/8/4/4 & 75/75 \\
subtle & design & worlds per scan class: \texttt{cutoff\_delivery} 15, \texttt{ineligible\_credit\_desc} 15, \texttt{personal\_expense} 15, \texttt{value\_alteration} 1 &  & pass \\
\bottomrule
\end{tabular}


==> tables/v22_scan_noise.tex <==
% auto-generated by scripts/build_v22_tables.py from results/v22/analysis.json — do not hand-edit (pool v22; hit/instances [exact 95% interval])
\begin{tabular}{llrrrr}
\toprule
arm & noise & \texttt{cutoff\_delivery} & \texttt{ineligible\_credit\_desc} & \texttt{personal\_expense} & \texttt{value\_alteration} \\
\midrule
\texttt{file\_as\_is} & clean & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] \\
\texttt{file\_as\_is} & mild\_scan & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] \\
\texttt{file\_as\_is} & noisy\_scan & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] \\
\texttt{flag\_everything} & clean & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] \\
\texttt{flag\_everything} & mild\_scan & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] \\
\texttt{flag\_everything} & noisy\_scan & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] \\
\texttt{malha\_rules} & clean & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] \\
\texttt{malha\_rules} & mild\_scan & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] \\
\texttt{malha\_rules} & noisy\_scan & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] \\
\texttt{ocr\_rules} & clean & 15/15 [0.78, 1.00] & 15/15 [0.78, 1.00] & 15/15 [0.78, 1.00] & 15/15 [0.78, 1.00] \\
\texttt{ocr\_rules} & mild\_scan & 15/15 [0.78, 1.00] & 6/15 [0.16, 0.68] & 15/15 [0.78, 1.00] & 7/15 [0.21, 0.73] \\
\texttt{ocr\_rules} & noisy\_scan & 15/15 [0.78, 1.00] & 7/15 [0.21, 0.73] & 15/15 [0.78, 1.00] & 3/15 [0.04, 0.48] \\
\texttt{malha\_rules\_book4} & clean & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] \\
\texttt{malha\_rules\_book4} & mild\_scan & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] \\
\texttt{malha\_rules\_book4} & noisy\_scan & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] & 0/15 [0.00, 0.22] \\
\texttt{ocr\_rules\_book4} & clean & 15/15 [0.78, 1.00] & 15/15 [0.78, 1.00] & 15/15 [0.78, 1.00] & 15/15 [0.78, 1.00] \\
\texttt{ocr\_rules\_book4} & mild\_scan & 15/15 [0.78, 1.00] & 6/15 [0.16, 0.68] & 15/15 [0.78, 1.00] & 7/15 [0.21, 0.73] \\
\texttt{ocr\_rules\_book4} & noisy\_scan & 15/15 [0.78, 1.00] & 7/15 [0.21, 0.73] & 15/15 [0.78, 1.00] & 3/15 [0.04, 0.48] \\
\texttt{ocr\_rules\_book4\_deskew} & clean & 15/15 [0.78, 1.00] & 10/15 [0.38, 0.88] & 15/15 [0.78, 1.00] & 0/15 [0.00, 0.22] \\
\texttt{ocr\_rules\_book4\_deskew} & mild\_scan & 15/15 [0.78, 1.00] & 10/15 [0.38, 0.88] & 15/15 [0.78, 1.00] & 12/15 [0.52, 0.96] \\
\texttt{ocr\_rules\_book4\_deskew} & noisy\_scan & 15/15 [0.78, 1.00] & 10/15 [0.38, 0.88] & 15/15 [0.78, 1.00] & 12/15 [0.52, 0.96] \\
\texttt{ocr\_rules\_book4\_vlm} & clean & not run & not run & not run & not run \\
\texttt{ocr\_rules\_book4\_vlm} & mild\_scan & not run & not run & not run & not run \\
\texttt{ocr\_rules\_book4\_vlm} & noisy\_scan & 15/15 [0.78, 1.00] & 15/15 [0.78, 1.00] & 15/15 [0.78, 1.00] & 15/15 [0.78, 1.00] \\
\texttt{agent\_v2\_fixed+glm-flash} & clean & 13/15 [0.60, 0.98] & 7/15 [0.21, 0.73] & 15/15 [0.78, 1.00] & 6/15 [0.16, 0.68] \\
\texttt{agent\_v2\_fixed+glm-flash} & mild\_scan & not run & not run & not run & not run \\
\texttt{agent\_v2\_fixed+glm-flash} & noisy\_scan & 14/15 [0.68, 1.00] & 3/15 [0.04, 0.48] & 14/15 [0.68, 1.00] & 4/15 [0.08, 0.55] \\
\texttt{agent\_v2\_vlm+glm-flash} & clean & not run & not run & not run & not run \\
\texttt{agent\_v2\_vlm+glm-flash} & mild\_scan & not run & not run & not run & not run \\
\texttt{agent\_v2\_vlm+glm-flash} & noisy\_scan & 13/15 [0.60, 0.98] & 2/15 [0.02, 0.40] & 15/15 [0.78, 1.00] & 5/15 [0.12, 0.62] \\
\texttt{agent\_v2\_vlm\_book4+glm-flash} & clean & not run & not run & not run & not run \\
\texttt{agent\_v2\_vlm\_book4+glm-flash} & mild\_scan & not run & not run & not run & not run \\
\texttt{agent\_v2\_vlm\_book4+glm-flash} & noisy\_scan & 15/15 [0.78, 1.00] & 10/15 [0.38, 0.88] & 15/15 [0.78, 1.00] & 9/15 [0.32, 0.84] \\
\texttt{ocr\_rules\_book4\_reocr} & clean & 15/15 [0.78, 1.00] & 6/15 [0.16, 0.68] & 15/15 [0.78, 1.00] & 15/15 [0.78, 1.00] \\
\texttt{ocr\_rules\_book4\_reocr} & mild\_scan & 15/15 [0.78, 1.00] & 6/15 [0.16, 0.68] & 15/15 [0.78, 1.00] & 7/15 [0.21, 0.73] \\
\texttt{ocr\_rules\_book4\_reocr} & noisy\_scan & 15/15 [0.78, 1.00] & 7/15 [0.21, 0.73] & 15/15 [0.78, 1.00] & 3/15 [0.04, 0.48] \\
\texttt{ocr\_rules\_deskew} & clean & 15/15 [0.78, 1.00] & 10/15 [0.38, 0.88] & 15/15 [0.78, 1.00] & 0/15 [0.00, 0.22] \\
\texttt{ocr\_rules\_deskew} & mild\_scan & 15/15 [0.78, 1.00] & 10/15 [0.38, 0.88] & 15/15 [0.78, 1.00] & 12/15 [0.52, 0.96] \\
\texttt{ocr\_rules\_deskew} & noisy\_scan & 15/15 [0.78, 1.00] & 10/15 [0.38, 0.88] & 15/15 [0.78, 1.00] & 12/15 [0.52, 0.96] \\
\texttt{ocr\_rules\_reocr} & clean & 15/15 [0.78, 1.00] & 6/15 [0.16, 0.68] & 15/15 [0.78, 1.00] & 15/15 [0.78, 1.00] \\
\texttt{ocr\_rules\_reocr} & mild\_scan & 15/15 [0.78, 1.00] & 6/15 [0.16, 0.68] & 15/15 [0.78, 1.00] & 7/15 [0.21, 0.73] \\
\texttt{ocr\_rules\_reocr} & noisy\_scan & 15/15 [0.78, 1.00] & 7/15 [0.21, 0.73] & 15/15 [0.78, 1.00] & 3/15 [0.04, 0.48] \\
\texttt{ocr\_rules\_vlm} & clean & not run & not run & not run & not run \\
\texttt{ocr\_rules\_vlm} & mild\_scan & not run & not run & not run & not run \\
\texttt{ocr\_rules\_vlm} & noisy\_scan & 15/15 [0.78, 1.00] & 15/15 [0.78, 1.00] & 15/15 [0.78, 1.00] & 15/15 [0.78, 1.00] \\
\bottomrule
\end{tabular}


==> tables/v22_sensitivity.tex <==
% auto-generated by scripts/build_v22_tables.py from results/v22/analysis.json — do not hand-edit (pool v22)
\begin{tabular}{lrrrrrr}
\toprule
contrast & conservative / R\$250 & conservative / R\$1500 & neutral / R\$250 & neutral / R\$1500 & aggressive / R\$250 & aggressive / R\$1500 \\
\midrule
\texttt{ocr\_rules\_book4} $-$ \texttt{agent\_v2\_vlm\_book4+glm-flash} (clean) & not run & not run & not run & not run & not run & not run \\
\texttt{agent\_v2\_vlm+glm-flash} $-$ \texttt{ocr\_rules\_book4\_vlm} (clean) & not run & not run & not run & not run & not run & not run \\
\texttt{agent\_v2\_fixed+glm-flash} $-$ \texttt{agent\_v2\_vlm+glm-flash} (clean) & not run & not run & not run & not run & not run & not run \\
\texttt{ocr\_rules\_book4\_reocr} $-$ \texttt{ocr\_rules\_book4\_deskew} (clean) & \textbf{-1,585 [-2,861, -594]} & \textbf{-1,585 [-2,861, -594]} & \textbf{-3,528 [-6,432, -1,278]} & \textbf{-3,528 [-6,432, -1,278]} & \textbf{-8,383 [-15,373, -2,971]} & \textbf{-8,383 [-15,373, -2,971]} \\
\texttt{ocr\_rules\_book4} $-$ \texttt{agent\_v2\_fixed+glm-flash} (clean) & \textbf{-2,749 [-4,038, -1,704]} & \textbf{-4,707 [-6,175, -3,487]} & \textbf{-6,452 [-9,470, -3,918]} & \textbf{-8,411 [-11,537, -5,802]} & \textbf{-15,711 [-23,083, -9,470]} & \textbf{-17,670 [-25,084, -11,387]} \\
\texttt{ocr\_rules\_book4} $-$ \texttt{agent\_v2\_vlm+glm-flash} (clean) & not run & not run & not run & not run & not run & not run \\
\texttt{ocr\_rules\_book4} $-$ \texttt{ocr\_rules\_book4\_vlm} (clean) & not run & not run & not run & not run & not run & not run \\
\texttt{ocr\_rules\_book4\_deskew} $-$ \texttt{ocr\_rules\_book4\_vlm} (clean) & not run & not run & not run & not run & not run & not run \\
\texttt{ocr\_rules\_book4\_reocr} $-$ \texttt{ocr\_rules\_book4} (clean) & \textbf{+358 [+136, +621]} & \textbf{+358 [+136, +621]} & \textbf{+1,074 [+408, +1,863]} & \textbf{+1,074 [+408, +1,863]} & \textbf{+2,864 [+1,089, +4,969]} & \textbf{+2,864 [+1,089, +4,969]} \\
\texttt{ocr\_rules\_book4\_deskew} $-$ \texttt{agent\_v2\_vlm\_book4+glm-flash} (clean) & not run & not run & not run & not run & not run & not run \\
\texttt{ocr\_rules\_book4\_vlm} $-$ \texttt{agent\_v2\_vlm\_book4+glm-flash} (clean) & not run & not run & not run & not run & not run & not run \\
\texttt{agent\_v2\_vlm+glm-flash} $-$ \texttt{agent\_v2\_vlm\_book4+glm-flash} (clean) & not run & not run & not run & not run & not run & not run \\
\texttt{malha\_rules} $-$ \texttt{ocr\_rules\_book4} (clean) & \textbf{+4,438 [+3,164, +5,852]} & \textbf{+4,438 [+3,164, +5,852]} & \textbf{+12,086 [+8,757, +15,681]} & \textbf{+12,086 [+8,757, +15,681]} & \textbf{+31,206 [+22,717, +40,369]} & \textbf{+31,206 [+22,717, +40,369]} \\
\texttt{malha\_rules} $-$ \texttt{agent\_v2\_vlm\_book4+glm-flash} (clean) & not run & not run & not run & not run & not run & not run \\
\texttt{malha\_rules\_book4} $-$ \texttt{ocr\_rules\_book4} (clean) & \textbf{+3,753 [+2,523, +5,179]} & \textbf{+3,753 [+2,523, +5,179]} & \textbf{+10,030 [+6,870, +13,573]} & \textbf{+10,030 [+6,870, +13,573]} & \textbf{+25,723 [+17,632, +34,630]} & \textbf{+25,723 [+17,632, +34,630]} \\
\texttt{ocr\_rules} $-$ \texttt{agent\_v2\_vlm+glm-flash} (clean) & not run & not run & not run & not run & not run & not run \\
\texttt{ocr\_rules} $-$ \texttt{agent\_v2\_fixed+glm-flash} (clean) & \textbf{-2,063 [-3,395, -972]} & \textbf{-4,022 [-5,557, -2,762]} & \textbf{-4,396 [-7,504, -1,764]} & \textbf{-6,355 [-9,573, -3,604]} & \textbf{-10,229 [-17,743, -3,685]} & \textbf{-12,187 [-19,807, -5,584]} \\
\texttt{malha\_rules} $-$ \texttt{agent\_v2\_vlm+glm-flash} (clean) & not run & not run & not run & not run & not run & not run \\
\texttt{malha\_rules} $-$ \texttt{agent\_v2\_fixed+glm-flash} (clean) & \textbf{+1,690 [+925, +2,508]} & -269 [-1,300, +766] & \textbf{+5,634 [+3,416, +7,998]} & \textbf{+3,676 [+1,330, +6,181]} & \textbf{+15,495 [+9,698, +21,713]} & \textbf{+13,536 [+7,604, +19,864]} \\
\texttt{ocr\_rules} $-$ \texttt{agent\_v2\_vlm\_book4+glm-flash} (clean) & not run & not run & not run & not run & not run & not run \\
\texttt{ocr\_rules\_book4\_deskew} $-$ \texttt{agent\_v2\_vlm+glm-flash} (clean) & not run & not run & not run & not run & not run & not run \\
\texttt{ocr\_rules\_book4\_deskew} $-$ \texttt{agent\_v2\_fixed+glm-flash} (clean) & \textbf{-805 [-1,416, -220]} & \textbf{-2,764 [-3,645, -1,919]} & \textbf{-1,851 [-3,577, -270]} & \textbf{-3,809 [-5,643, -2,068]} & \textbf{-4,464 [-9,017, -314]} & \textbf{-6,423 [-10,998, -2,248]} \\
\texttt{ocr\_rules\_book4\_vlm} $-$ \texttt{agent\_v2\_fixed+glm-flash} (clean) & not run & not run & not run & not run & not run & not run \\
\texttt{ocr\_rules\_book4} $-$ \texttt{agent\_v2\_vlm\_book4+glm-flash} (mild\_scan) & not run & not run & not run & not run & not run & not run \\
\texttt{agent\_v2\_vlm+glm-flash} $-$ \texttt{ocr\_rules\_book4\_vlm} (mild\_scan) & not run & not run & not run & not run & not run & not run \\
\texttt{agent\_v2\_fixed+glm-flash} $-$ \texttt{agent\_v2\_vlm+glm-flash} (mild\_scan) & not run & not run & not run & not run & not run & not run \\
\texttt{ocr\_rules\_book4\_reocr} $-$ \texttt{ocr\_rules\_book4\_deskew} (mild\_scan) & \textbf{+1,021 [+238, +1,978]} & \textbf{+1,021 [+238, +1,978]} & \textbf{+2,395 [+594, +4,613]} & \textbf{+2,395 [+594, +4,613]} & \textbf{+5,831 [+1,473, +11,192]} & \textbf{+5,831 [+1,473, +11,192]} \\
\texttt{ocr\_rules\_book4} $-$ \texttt{agent\_v2\_fixed+glm-flash} (mild\_scan) & not run & not run & not run & not run & not run & not run \\
\texttt{ocr\_rules\_book4} $-$ \texttt{agent\_v2\_vlm+glm-flash} (mild\_scan) & not run & not run & not run & not run & not run & not run \\
\texttt{ocr\_rules\_book4} $-$ \texttt{ocr\_rules\_book4\_vlm} (mild\_scan) & not run & not run & not run & not run & not run & not run \\
\texttt{ocr\_rules\_book4\_deskew} $-$ \texttt{ocr\_rules\_book4\_vlm} (mild\_scan) & not run & not run & not run & not run & not run & not run \\
\texttt{ocr\_rules\_book4\_reocr} $-$ \texttt{ocr\_rules\_book4} (mild\_scan) & +0 [+0, +0] & +0 [+0, +0] & +0 [+0, +0] & +0 [+0, +0] & +0 [+0, +0] & +0 [+0, +0] \\
\texttt{ocr\_rules\_book4\_deskew} $-$ \texttt{agent\_v2\_vlm\_book4+glm-flash} (mild\_scan) & not run & not run & not run & not run & not run & not run \\
\texttt{ocr\_rules\_book4\_vlm} $-$ \texttt{agent\_v2\_vlm\_book4+glm-flash} (mild\_scan) & not run & not run & not run & not run & not run & not run \\
\texttt{agent\_v2\_vlm+glm-flash} $-$ \texttt{agent\_v2\_vlm\_book4+glm-flash} (mild\_scan) & not run & not run & not run & not run & not run & not run \\
\texttt{malha\_rules} $-$ \texttt{ocr\_rules\_book4} (mild\_scan) & \textbf{+3,028 [+1,975, +4,263]} & \textbf{+3,028 [+1,975, +4,263]} & \textbf{+8,622 [+5,752, +11,852]} & \textbf{+8,622 [+5,752, +11,852]} & \textbf{+22,605 [+15,165, +30,934]} & \textbf{+22,605 [+15,165, +30,934]} \\
\texttt{malha\_rules} $-$ \texttt{agent\_v2\_vlm\_book4+glm-flash} (mild\_scan) & not run & not run & not run & not run & not run & not run \\
\texttt{malha\_rules\_book4} $-$ \texttt{ocr\_rules\_book4} (mild\_scan) & \textbf{+2,343 [+1,395, +3,518]} & \textbf{+2,343 [+1,395, +3,518]} & \textbf{+6,566 [+4,001, +9,544]} & \textbf{+6,566 [+4,001, +9,544]} & \textbf{+17,122 [+10,477, +24,636]} & \textbf{+17,122 [+10,477, +24,636]} \\
\texttt{ocr\_rules} $-$ \texttt{agent\_v2\_vlm+glm-flash} (mild\_scan) & not run & not run & not run & not run & not run & not run \\
\texttt{ocr\_rules} $-$ \texttt{agent\_v2\_fixed+glm-flash} (mild\_scan) & not run & not run & not run & not run & not run & not run \\
\texttt{malha\_rules} $-$ \texttt{agent\_v2\_vlm+glm-flash} (mild\_scan) & not run & not run & not run & not run & not run & not run \\
\texttt{malha\_rules} $-$ \texttt{agent\_v2\_fixed+glm-flash} (mild\_scan) & not run & not run & not run & not run & not run & not run \\
\texttt{ocr\_rules} $-$ \texttt{agent\_v2\_vlm\_book4+glm-flash} (mild\_scan) & not run & not run & not run & not run & not run & not run \\
\texttt{ocr\_rules\_book4\_deskew} $-$ \texttt{agent\_v2\_vlm+glm-flash} (mild\_scan) & not run & not run & not run & not run & not run & not run \\
\texttt{ocr\_rules\_book4\_deskew} $-$ \texttt{agent\_v2\_fixed+glm-flash} (mild\_scan) & not run & not run & not run & not run & not run & not run \\
\texttt{ocr\_rules\_book4\_vlm} $-$ \texttt{agent\_v2\_fixed+glm-flash} (mild\_scan) & not run & not run & not run & not run & not run & not run \\
\texttt{ocr\_rules\_book4} $-$ \texttt{agent\_v2\_vlm\_book4+glm-flash} (noisy\_scan) & -33 [-366, +365] & \textbf{-2,595 [-3,308, -1,861]} & +679 [-95, +1,609] & \textbf{-1,883 [-2,917, -725]} & \textbf{+2,460 [+563, +4,747]} & -103 [-2,163, +2,348] \\
\texttt{agent\_v2\_vlm+glm-flash} $-$ \texttt{ocr\_rules\_book4\_vlm} (noisy\_scan) & \textbf{+2,803 [+1,754, +4,063]} & \textbf{+4,761 [+3,598, +6,097]} & \textbf{+6,777 [+4,155, +9,851]} & \textbf{+8,735 [+6,035, +11,874]} & \textbf{+16,710 [+10,143, +24,422]} & \textbf{+18,668 [+12,055, +26,408]} \\
\texttt{agent\_v2\_fixed+glm-flash} $-$ \texttt{agent\_v2\_vlm+glm-flash} (noisy\_scan) & +45 [-758, +930] & -351 [-1,445, +775] & +40 [-2,070, +2,212] & -356 [-2,680, +2,020] & +26 [-5,381, +5,439] & -369 [-5,969, +5,191] \\
\texttt{ocr\_rules\_book4\_reocr} $-$ \texttt{ocr\_rules\_book4\_deskew} (noisy\_scan) & \textbf{+1,093 [+420, +1,934]} & \textbf{+1,406 [+699, +2,263]} & \textbf{+2,456 [+919, +4,370]} & \textbf{+2,768 [+1,221, +4,681]} & \textbf{+5,861 [+2,170, +10,461]} & \textbf{+6,174 [+2,463, +10,753]} \\
\texttt{ocr\_rules\_book4} $-$ \texttt{agent\_v2\_fixed+glm-flash} (noisy\_scan) & \textbf{-1,230 [-2,320, -427]} & \textbf{-2,480 [-3,670, -1,515]} & \textbf{-2,983 [-5,589, -972]} & \textbf{-4,233 [-6,914, -2,107]} & \textbf{-7,367 [-13,773, -2,328]} & \textbf{-8,617 [-15,042, -3,492]} \\
\texttt{ocr\_rules\_book4} $-$ \texttt{agent\_v2\_vlm+glm-flash} (noisy\_scan) & \textbf{-1,185 [-2,428, -96]} & \textbf{-2,831 [-4,174, -1,621]} & \textbf{-2,944 [-5,981, -258]} & \textbf{-4,590 [-7,706, -1,829]} & \textbf{-7,340 [-14,939, -597]} & \textbf{-8,986 [-16,633, -2,206]} \\
\texttt{ocr\_rules\_book4} $-$ \texttt{ocr\_rules\_book4\_vlm} (noisy\_scan) & \textbf{+1,618 [+861, +2,529]} & \textbf{+1,930 [+1,146, +2,855]} & \textbf{+3,833 [+2,063, +5,931]} & \textbf{+4,145 [+2,360, +6,265]} & \textbf{+9,370 [+5,045, +14,465]} & \textbf{+9,682 [+5,351, +14,770]} \\
\texttt{ocr\_rules\_book4\_deskew} $-$ \texttt{ocr\_rules\_book4\_vlm} (noisy\_scan) & \textbf{+525 [+151, +992]} & \textbf{+525 [+151, +992]} & \textbf{+1,377 [+414, +2,533]} & \textbf{+1,377 [+414, +2,533]} & \textbf{+3,508 [+1,086, +6,391]} & \textbf{+3,508 [+1,086, +6,391]} \\
\texttt{ocr\_rules\_book4\_reocr} $-$ \texttt{ocr\_rules\_book4} (noisy\_scan) & +0 [+0, +0] & +0 [+0, +0] & +0 [+0, +0] & +0 [+0, +0] & +0 [+0, +0] & +0 [+0, +0] \\
\texttt{ocr\_rules\_book4\_deskew} $-$ \texttt{agent\_v2\_vlm\_book4+glm-flash} (noisy\_scan) & \textbf{-1,126 [-1,958, -466]} & \textbf{-4,001 [-4,949, -3,120]} & \textbf{-1,776 [-3,728, -227]} & \textbf{-4,651 [-6,585, -2,963]} & -3,402 [-8,160, +415] & \textbf{-6,277 [-10,972, -2,388]} \\
\texttt{ocr\_rules\_book4\_vlm} $-$ \texttt{agent\_v2\_vlm\_book4+glm-flash} (noisy\_scan) & \textbf{-1,651 [-2,518, -942]} & \textbf{-4,526 [-5,500, -3,621]} & \textbf{-3,153 [-5,167, -1,513]} & \textbf{-6,028 [-8,055, -4,294]} & \textbf{-6,910 [-11,779, -2,947]} & \textbf{-9,785 [-14,618, -5,799]} \\
\texttt{agent\_v2\_vlm+glm-flash} $-$ \texttt{agent\_v2\_vlm\_book4+glm-flash} (noisy\_scan) & \textbf{+1,152 [+25, +2,448]} & +236 [-1,051, +1,685] & \textbf{+3,623 [+800, +6,764]} & +2,707 [-160, +5,931] & \textbf{+9,800 [+2,700, +17,643]} & \textbf{+8,884 [+1,838, +16,778]} \\
\texttt{malha\_rules} $-$ \texttt{ocr\_rules\_book4} (noisy\_scan) & \textbf{+2,820 [+1,782, +4,068]} & \textbf{+2,508 [+1,449, +3,767]} & \textbf{+8,254 [+5,395, +11,543]} & \textbf{+7,941 [+5,058, +11,228]} & \textbf{+21,836 [+14,353, +30,237]} & \textbf{+21,524 [+14,052, +29,888]} \\
\texttt{malha\_rules} $-$ \texttt{agent\_v2\_vlm\_book4+glm-flash} (noisy\_scan) & \textbf{+2,787 [+1,710, +4,061]} & -88 [-1,334, +1,337] & \textbf{+8,933 [+6,007, +12,247]} & \textbf{+6,058 [+3,060, +9,445]} & \textbf{+24,296 [+16,728, +32,811]} & \textbf{+21,421 [+13,785, +29,959]} \\
\texttt{malha\_rules\_book4} $-$ \texttt{ocr\_rules\_book4} (noisy\_scan) & \textbf{+2,135 [+1,191, +3,316]} & \textbf{+1,823 [+862, +3,018]} & \textbf{+6,197 [+3,655, +9,206]} & \textbf{+5,885 [+3,328, +8,904]} & \textbf{+16,354 [+9,814, +23,964]} & \textbf{+16,041 [+9,469, +23,679]} \\
\texttt{ocr\_rules} $-$ \texttt{agent\_v2\_vlm+glm-flash} (noisy\_scan) & -500 [-1,752, +598] & \textbf{-2,146 [-3,455, -944]} & -888 [-3,896, +1,824] & -2,534 [-5,584, +220] & -1,858 [-9,335, +4,910] & -3,504 [-11,031, +3,296] \\
\texttt{ocr\_rules} $-$ \texttt{agent\_v2\_fixed+glm-flash} (noisy\_scan) & -545 [-1,657, +273] & \textbf{-1,795 [-2,991, -812]} & -927 [-3,533, +1,145] & -2,177 [-4,868, +4] & -1,884 [-8,227, +3,317] & -3,134 [-9,585, +2,178] \\
\texttt{malha\_rules} $-$ \texttt{agent\_v2\_vlm+glm-flash} (noisy\_scan) & \textbf{+1,635 [+826, +2,554]} & -323 [-1,316, +734] & \textbf{+5,310 [+3,099, +7,766]} & \textbf{+3,351 [+1,014, +5,907]} & \textbf{+14,496 [+8,769, +20,817]} & \textbf{+12,538 [+6,725, +18,994]} \\
\texttt{malha\_rules} $-$ \texttt{agent\_v2\_fixed+glm-flash} (noisy\_scan) & \textbf{+1,590 [+826, +2,408]} & +28 [-878, +967] & \textbf{+5,270 [+3,034, +7,676]} & \textbf{+3,708 [+1,379, +6,206]} & \textbf{+14,469 [+8,581, +20,868]} & \textbf{+12,907 [+6,941, +19,359]} \\
\texttt{ocr\_rules} $-$ \texttt{agent\_v2\_vlm\_book4+glm-flash} (noisy\_scan) & \textbf{+652 [+125, +1,263]} & \textbf{-1,910 [-2,715, -1,079]} & \textbf{+2,735 [+1,296, +4,428]} & +173 [-1,420, +1,951] & \textbf{+7,942 [+4,151, +12,401]} & \textbf{+5,380 [+1,551, +9,871]} \\
\texttt{ocr\_rules\_book4\_deskew} $-$ \texttt{agent\_v2\_vlm+glm-flash} (noisy\_scan) & \textbf{-2,279 [-3,555, -1,176]} & \textbf{-4,237 [-5,606, -2,998]} & \textbf{-5,400 [-8,492, -2,674]} & \textbf{-7,358 [-10,533, -4,523]} & \textbf{-13,202 [-20,936, -6,389]} & \textbf{-15,160 [-23,004, -8,226]} \\
\texttt{ocr\_rules\_book4\_deskew} $-$ \texttt{agent\_v2\_fixed+glm-flash} (noisy\_scan) & \textbf{-2,323 [-3,608, -1,267]} & \textbf{-3,886 [-5,244, -2,714]} & \textbf{-5,439 [-8,458, -2,881]} & \textbf{-7,002 [-10,096, -4,353]} & \textbf{-13,228 [-20,608, -6,886]} & \textbf{-14,791 [-22,235, -8,348]} \\
\texttt{ocr\_rules\_book4\_vlm} $-$ \texttt{agent\_v2\_fixed+glm-flash} (noisy\_scan) & \textbf{-2,848 [-4,204, -1,763]} & \textbf{-4,410 [-5,837, -3,218]} & \textbf{-6,816 [-9,989, -4,221]} & \textbf{-8,379 [-11,622, -5,698]} & \textbf{-16,737 [-24,464, -10,307]} & \textbf{-18,299 [-26,104, -11,772]} \\
\bottomrule
\end{tabular}


==> tables/v22_strict_citation.tex <==
% auto-generated by scripts/build_v22_tables.py from results/v22/analysis.json — do not hand-edit (pool v22, mean EL (BRL), neutral_r250)
\begin{tabular}{llrrrr}
\toprule
arm & noise & permissive & strict & strict\_cap3 & strict\_cap1 \\
\midrule
\texttt{file\_as\_is} & clean & 26,430 & 26,430 & 26,430 & 26,430 \\
\texttt{file\_as\_is} & mild\_scan & 26,430 & 26,430 & 26,430 & 26,430 \\
\texttt{file\_as\_is} & noisy\_scan & 26,430 & 26,430 & 26,430 & 26,430 \\
\texttt{flag\_everything} & clean & 31,180 & 31,180 & 31,180 & 31,180 \\
\texttt{flag\_everything} & mild\_scan & 31,180 & 31,180 & 31,180 & 31,180 \\
\texttt{flag\_everything} & noisy\_scan & 31,180 & 31,180 & 31,180 & 31,180 \\
\texttt{malha\_rules} & clean & 12,768 & 12,768 & 12,768 & 12,768 \\
\texttt{malha\_rules} & mild\_scan & 12,768 & 12,768 & 12,768 & 12,768 \\
\texttt{malha\_rules} & noisy\_scan & 12,768 & 12,768 & 12,768 & 12,768 \\
\texttt{ocr\_rules} & clean & 2,738 & 2,738 & 2,738 & 2,738 \\
\texttt{ocr\_rules} & mild\_scan & 6,202 & 6,202 & 6,202 & 6,202 \\
\texttt{ocr\_rules} & noisy\_scan & 6,571 & 6,571 & 6,571 & 6,571 \\
\texttt{malha\_rules\_book4} & clean & 10,712 & 10,712 & 10,712 & 10,712 \\
\texttt{malha\_rules\_book4} & mild\_scan & 10,712 & 10,712 & 10,712 & 10,712 \\
\texttt{malha\_rules\_book4} & noisy\_scan & 10,712 & 10,712 & 10,712 & 10,712 \\
\texttt{ocr\_rules\_book4} & clean & 682 & 682 & 682 & 682 \\
\texttt{ocr\_rules\_book4} & mild\_scan & 4,146 & 4,146 & 4,146 & 4,146 \\
\texttt{ocr\_rules\_book4} & noisy\_scan & 4,514 & 4,514 & 4,514 & 4,514 \\
\texttt{ocr\_rules\_book4\_deskew} & clean & 5,283 & 5,283 & 5,283 & 5,283 \\
\texttt{ocr\_rules\_book4\_deskew} & mild\_scan & 1,751 & 1,751 & 1,751 & 1,751 \\
\texttt{ocr\_rules\_book4\_deskew} & noisy\_scan & 2,059 & 2,059 & 2,059 & 2,059 \\
\texttt{ocr\_rules\_book4\_vlm} & clean & not run & not run & not run & not run \\
\texttt{ocr\_rules\_book4\_vlm} & mild\_scan & not run & not run & not run & not run \\
\texttt{ocr\_rules\_book4\_vlm} & noisy\_scan & 682 & 682 & 682 & 682 \\
\texttt{agent\_v2\_fixed+glm-flash} & clean & 7,134 & 7,150 & 7,150 & 7,305 \\
\texttt{agent\_v2\_fixed+glm-flash} & mild\_scan & not run & not run & not run & not run \\
\texttt{agent\_v2\_fixed+glm-flash} & noisy\_scan & 7,498 & 7,527 & 7,527 & 7,597 \\
\texttt{agent\_v2\_vlm+glm-flash} & clean & not run & not run & not run & not run \\
\texttt{agent\_v2\_vlm+glm-flash} & mild\_scan & not run & not run & not run & not run \\
\texttt{agent\_v2\_vlm+glm-flash} & noisy\_scan & 7,458 & 7,508 & 7,508 & 7,563 \\
\texttt{agent\_v2\_vlm\_book4+glm-flash} & clean & not run & not run & not run & not run \\
\texttt{agent\_v2\_vlm\_book4+glm-flash} & mild\_scan & not run & not run & not run & not run \\
\texttt{agent\_v2\_vlm\_book4+glm-flash} & noisy\_scan & 3,835 & 3,835 & 3,835 & 3,835 \\
\texttt{ocr\_rules\_book4\_reocr} & clean & 1,756 & 1,756 & 1,756 & 1,756 \\
\texttt{ocr\_rules\_book4\_reocr} & mild\_scan & 4,146 & 4,146 & 4,146 & 4,146 \\
\texttt{ocr\_rules\_book4\_reocr} & noisy\_scan & 4,514 & 4,514 & 4,514 & 4,514 \\
\texttt{ocr\_rules\_deskew} & clean & 7,339 & 7,339 & 7,339 & 7,339 \\
\texttt{ocr\_rules\_deskew} & mild\_scan & 3,807 & 3,807 & 3,807 & 3,807 \\
\texttt{ocr\_rules\_deskew} & noisy\_scan & 4,115 & 4,115 & 4,115 & 4,115 \\
\texttt{ocr\_rules\_reocr} & clean & 3,812 & 3,812 & 3,812 & 3,812 \\
\texttt{ocr\_rules\_reocr} & mild\_scan & 6,202 & 6,202 & 6,202 & 6,202 \\
\texttt{ocr\_rules\_reocr} & noisy\_scan & 6,571 & 6,571 & 6,571 & 6,571 \\
\texttt{ocr\_rules\_vlm} & clean & not run & not run & not run & not run \\
\texttt{ocr\_rules\_vlm} & mild\_scan & not run & not run & not run & not run \\
\texttt{ocr\_rules\_vlm} & noisy\_scan & 2,738 & 2,738 & 2,738 & 2,738 \\
\bottomrule
\end{tabular}


==> tables/v22_subtle.tex <==
% auto-generated by scripts/build_v22_tables.py from results/v22/analysis.json — do not hand-edit (pool v22_subtle; date = date-format change, sem. = semantic rewording (PRE-REGISTRATION-V3 s.9.1), orig. = wording unchanged)
\begin{tabular}{llrrrrrrr}
\toprule
arm & noise & mean EL (BRL) & \texttt{ocr\_rules\_book4} $-$ arm [95\% CI] & \texttt{cutoff\_delivery} (date) & \texttt{personal\_expense} (sem.) & \texttt{ineligible\_credit\_desc} (sem.) & \texttt{expense\_personal\_mixed} (sem.) & \texttt{value\_alteration} (orig.) \\
\midrule
\texttt{file\_as\_is} & clean & 23,617 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 0/1 \\
\texttt{file\_as\_is} & mild\_scan & 23,617 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 0/1 \\
\texttt{file\_as\_is} & noisy\_scan & 23,617 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 0/1 \\
\texttt{flag\_everything} & clean & 28,367 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 0/1 \\
\texttt{flag\_everything} & mild\_scan & 28,367 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 0/1 \\
\texttt{flag\_everything} & noisy\_scan & 28,367 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 0/1 \\
\texttt{malha\_rules} & clean & 17,230 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 0/1 \\
\texttt{malha\_rules} & mild\_scan & 17,230 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 0/1 \\
\texttt{malha\_rules} & noisy\_scan & 17,230 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 0/1 \\
\texttt{ocr\_rules} & clean & 16,713 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 1/1 \\
\texttt{ocr\_rules} & mild\_scan & 16,713 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 1/1 \\
\texttt{ocr\_rules} & noisy\_scan & 17,297 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 0/1 \\
\texttt{malha\_rules\_book4} & clean & 15,942 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 0/1 \\
\texttt{malha\_rules\_book4} & mild\_scan & 15,942 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 0/1 \\
\texttt{malha\_rules\_book4} & noisy\_scan & 15,942 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 0/1 \\
\texttt{ocr\_rules\_book4} & clean & 15,426 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 1/1 \\
\texttt{ocr\_rules\_book4} & mild\_scan & 15,426 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 1/1 \\
\texttt{ocr\_rules\_book4} & noisy\_scan & 16,009 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 0/1 \\
\texttt{ocr\_rules\_book4\_deskew} & clean & 15,942 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 0/1 \\
\texttt{ocr\_rules\_book4\_deskew} & mild\_scan & 15,426 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 1/1 \\
\texttt{ocr\_rules\_book4\_deskew} & noisy\_scan & 15,426 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 1/1 \\
\texttt{ocr\_rules\_book4\_vlm} & clean & not run & -- & -- & -- & -- & -- & -- \\
\texttt{ocr\_rules\_book4\_vlm} & mild\_scan & 15,426 & +0 [+0, +0] & 0/15 & 0/15 & 0/15 & 0/15 & 1/1 \\
\texttt{ocr\_rules\_book4\_vlm} & noisy\_scan & not run & -- & -- & -- & -- & -- & -- \\
\texttt{agent\_v2\_fixed+glm-flash} & clean & 7,912 & \textbf{+7,514 [+3,481, +11,841]} & 15/15 & 14/15 & 4/15 & 2/15 & 0/1 \\
\texttt{agent\_v2\_fixed+glm-flash} & mild\_scan & not run & -- & -- & -- & -- & -- & -- \\
\texttt{agent\_v2\_fixed+glm-flash} & noisy\_scan & not run & -- & -- & -- & -- & -- & -- \\
\texttt{agent\_v2\_vlm+glm-flash} & clean & not run & -- & -- & -- & -- & -- & -- \\
\texttt{agent\_v2\_vlm+glm-flash} & mild\_scan & not run & -- & -- & -- & -- & -- & -- \\
\texttt{agent\_v2\_vlm+glm-flash} & noisy\_scan & not run & -- & -- & -- & -- & -- & -- \\
\texttt{agent\_v2\_vlm\_book4+glm-flash} & clean & not run & -- & -- & -- & -- & -- & -- \\
\texttt{agent\_v2\_vlm\_book4+glm-flash} & mild\_scan & not run & -- & -- & -- & -- & -- & -- \\
\texttt{agent\_v2\_vlm\_book4+glm-flash} & noisy\_scan & not run & -- & -- & -- & -- & -- & -- \\
\texttt{ocr\_rules\_book4\_reocr} & clean & 15,426 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 1/1 \\
\texttt{ocr\_rules\_book4\_reocr} & mild\_scan & 15,426 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 1/1 \\
\texttt{ocr\_rules\_book4\_reocr} & noisy\_scan & 16,009 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 0/1 \\
\texttt{ocr\_rules\_deskew} & clean & 17,230 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 0/1 \\
\texttt{ocr\_rules\_deskew} & mild\_scan & 16,713 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 1/1 \\
\texttt{ocr\_rules\_deskew} & noisy\_scan & 16,713 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 1/1 \\
\texttt{ocr\_rules\_reocr} & clean & 16,713 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 1/1 \\
\texttt{ocr\_rules\_reocr} & mild\_scan & 16,713 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 1/1 \\
\texttt{ocr\_rules\_reocr} & noisy\_scan & 17,297 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 0/1 \\
\texttt{ocr\_rules\_vlm} & clean & not run & -- & -- & -- & -- & -- & -- \\
\texttt{ocr\_rules\_vlm} & mild\_scan & 16,713 & -- & 0/15 & 0/15 & 0/15 & 0/15 & 1/1 \\
\texttt{ocr\_rules\_vlm} & noisy\_scan & not run & -- & -- & -- & -- & -- & -- \\
\bottomrule
\end{tabular}

